Neural Motion Blending Across Arbitrary Character Topologies

Motion blending in character animation enables the synthesis of new motions by interpolating between existing examples. Current methods are typically restricted to fixed skeleton topologies, requiring identical or near-identical skeletal structures across characters. We present a novel framework for motion blending across heterogeneous skeletons. The proposed architecture combines a semantic encoder, which extracts per-frame latent representations of the motion state, with a diffusion-based decoder, which reconstructs character-specific motion conditioned on this latent code. At inference, blended motions are obtained by interpolating the latent representations of two input motions. We train and evaluate the method on the Truebones Zoo dataset using motions defined on both same and distinct skeleton topologies, demonstrating the ability to achieve smooth and plausible blending in a variety of scenarios.

==> figures/retargeting_all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{media/qualitative/transfer_many.pdf}
    \caption{\textbf{Qualitative results: (C) Retargeting.}}
    \label{fig:xskel}
\end{figure}

==> tables/ablations_alpha.tex <==
\begin{table}[ht]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{3pt}
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabularx}{1.0\textwidth}{@{}lYYYY@{}}
\toprule
\mbox{\textbf{$\alpha(n)$}} &
\mbox{\textbf{FID $\downarrow$}} &
\mbox{\textbf{Proximity $\downarrow$}} &
\mbox{\textbf{Jerk Ratio $\sim 1$}} &
\mbox{\textbf{IntraDivDiff $\downarrow$}} \\
\midrule
Linear &
\cellcolor{secondgreen}$9.7607\ (9.2765) \pm 0.6020$ &
\cellcolor{bestgreen}$0.1203 \pm 0.0640$ &
\cellcolor{bestgreen}$1.4795 \pm 0.7121$ &
$0.1135 \pm 0.0697$ \\
Ease (1.0) &
\cellcolor{bestgreen}$9.7521\ (8.9828) \pm 0.6176$ &
\cellcolor{secondgreen}$0.1207 \pm 0.0632$ &
\cellcolor{secondgreen}$1.6469 \pm 0.8759$ &
\cellcolor{secondgreen}$0.1090 \pm 0.0687$ \\
Ease (2.0) &
$9.7816\ (9.0403) \pm 0.6333$ &
$0.1216 \pm 0.0638$ &
$1.7996 \pm 1.0100$ &
\cellcolor{bestgreen}$0.1047 \pm 0.0663$ \\
\bottomrule
\end{tabularx}%
}
\renewcommand{\arraystretch}{1}
\end{table}

==> tables/ablations_features.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}[htbp]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{3pt}
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabularx}{1.12\textwidth}{@{}lYYYY@{}}
\toprule
\textbf{In-Feats} &
\mbox{\textbf{FID $\downarrow$}} &
\mbox{\textbf{Proximity $\downarrow$}} &
\mbox{\textbf{Jerk Ratio $\sim 1$}} &
\mbox{\textbf{IntraDivDiff $\downarrow$}} \\
\midrule
Vel &
$10.7159 \pm 0.6496$ &
$0.1294 \pm 0.0649$ &
$2.5886 \pm 4.3425$ &
\cellcolor{secondgreen}$0.11 \pm 0.07$ \\
Rot &
\cellcolor{secondgreen}$10.63 \pm 0.66$ &
\cellcolor{secondgreen}$0.13 \pm 0.07$ &
\cellcolor{secondgreen}$1.81 \pm 1.28$ &
$0.11 \pm 0.07$ \\
Full &
\cellcolor{bestgreen}$9.75 \pm 0.62$ &
\cellcolor{bestgreen}$0.12 \pm 0.06$ &
\cellcolor{bestgreen}$1.65 \pm 0.88$ &
\cellcolor{bestgreen}$0.11 \pm 0.07$ \\
\bottomrule
\end{tabularx}%
}
\renewcommand{\arraystretch}{1}
\end{table}
